The impact of an employee's psychological contract breach on compliance with information security policies: intrinsic and extrinsic motivation

Despite the rapid rise in social engineering attacks, not all employees are as compliant with information security policies (ISPs) to the extent that organisations expect them to be. ISP non-compliance is caused by a variety of psychological motivation. This study investigates the effect of psychological contract breach (PCB) of employees on ISP compliance intention (ICI) by dividing them into intrinsic and extrinsic motivation using the theory of planned behaviour (TPB) and the general deterrence theory (GDT). Data analysis from UK employees (\textit{n=206}) showed that the higher the PCB, the lower the ICI. The study also found that PCBs significantly reduced intrinsic motivation (attitude and perceived fairness) for ICI, whereas PCBs did not moderate the relationship between extrinsic motivation (sanction severity and sanctions certainty) and ICI. As a result, this study successfully addresses the risks of PCBs in the field of IS security and proposes effective solutions for employees with high PCBs.

==> Acknowledgements.tex <==
\\
\vspace*{0.5cm}

I completed this research thanks to a lot of support and assistance from the following people.\\

First, thanks to my supervisor, Dr Nadine Michaelides, for providing guidance, sophisticated critique, connection to the partner company, and encouragement. Without her supervision and encouragement, I would not have been able to complete a dissertation of this quality. I would also like to thank Dr Harjinder Lallie, a course leader, for helping me publish my research as a quality journal article. Their contributions supported me to get through my master’s degree.\\

Furthermore, I would like to thank my anonymous contributor, a multinational industrial goods and services company. In particular, I cannot thank enough the CISO and two stakeholders of the company, who supported random sampling and survey distribution to their employees to conduct surveys anonymously and confidentially. I am also grateful for the over 260 employees of the company who participated in my online questionnaire. Thank you for taking your valuable time to participate in this thesis.\\

Finally, my appreciation goes to my friends and family for not only being involved in the pilot testing of my study, but also supporting me emotionally and mentally as always.
\clearpage
